The QCET Taxonomy of Standard Quality Criterion Names and Definitions for the Evaluation of NLP Systems

Prior work has shown that two NLP evaluation experiments that report results for the same quality criterion name (e.g. Fluency) do not necessarily evaluate the same aspect of quality, and the comparability implied by the name can be misleading. Not knowing when two evaluations are comparable in this sense means we currently lack the ability to draw reliable conclusions about system quality on the basis of multiple, independently conducted evaluations. This in turn hampers the ability of the field to progress scientifically as a whole, a pervasive issue in NLP since its beginning (Sparck Jones, 1981). It is hard to see how the issue of unclear comparability can be fully addressed other than by the creation of a standard set of quality criterion names and definitions that the several hundred quality criterion names actually in use in the field can be mapped to, and grounded in. Taking a strictly descriptive approach, the QCET Quality Criteria for Evaluation Taxonomy derives a standard set of quality criterion names and definitions from three surveys of evaluations reported in NLP, and structures them into a hierarchy where each parent node captures common aspects of its child nodes. We present QCET and the resources it consists of, and discuss its three main uses in (i) establishing comparability of existing evaluations, (ii) guiding the design of new evaluations, and (iii) assessing regulatory compliance.

==> latex/definition_templates.tex <==
\newcommand{\phhl}[1]{\sethlcolor{green!10}\hl{\textsf{\small #1}}\sethlcolor{yellow}}

\begin{table*}[ht]
    \centering\small
    \begin{tabular}{|p{0.9\textwidth}|}
    \hline
\textit{A better system... }\\
    \hline
    \hline
...is more \phhl{\$property}, where compared systems differ only in their outputs \\
    \hline
...produces \phhl{\$output\_type}s with fewer \phhl{\$error\_type}s \\
    \hline
...produces \phhl{\$output\_type}s with fewer \phhl{\$error\_type}s relative to the input\\
    \hline
...produces \phhl{\$output\_type}s that lack fewer of the \phhl{\$control\_attribute}s provided in the input \\
    \hline
...produces \phhl{\$output\_type}s with \phhl{\$\{more, less\}} \phhl{\$property} \phhl{*\$\{in their form, in their content/meaning, overall\}} \phhl{*\$additional\_constraint} \\
    \hline
...produces \phhl{\$output\_type}s that are \phhl{\$\{more, less\}} \phhl{\$property} \phhl{*\$\{in their form, in their content/meaning, overall\}} \phhl{*\$additional\_constraint} \\
    \hline
...produces \phhl{\$output\_type}s that are \phhl{\$\{more, less\}} \phhl{\$property} relative to the input \phhl{*\$additional\_constraint} \\
    \hline
...produces \phhl{\$output\_type}s of the input with fewer \phhl{\$error\_type}s \\
    \hline
...produces \phhl{\$output\_type}s that \phhl{*\$\{in their form, in their content/meaning, overall\}} less often differ from the given target \phhl{\$output\_type}s \phhl{*\$additional\_constraint} \\
    \hline
...produces \phhl{\$output\_type}s that are \phhl{*\$\{in their form, in their content/meaning, overall\}} more at the target level of \phhl{\$property} provided in the input \\
    \hline
...produces \phhl{\$output\_type}s that are \phhl{*\$\{in their form, in their content/meaning, overall\}} more similar to given target \phhl{\$output\_type}s \phhl{*\$additional\_constraint} \\
    \hline
...produces \phhl{\$output\_type}s that are \phhl{*\$\{in their form, in their content/meaning, overall\}} either (a) more \phhl{\$property}, or (b) less \phhl{\$property} \\
    \hline
...produces \phhl{\$output\_type}s that are \phhl{*\$\{in their form, in their content/meaning, overall\}} (a) more \phhl{\$property}, (b) less \phhl{\$property}, or (c) more at the target level of \phhl{\$property} provided in the input \phhl{*\$additional\_constraint} \\
    \hline
...produces \phhl{\$output\_type}s that \phhl{\$affect} \phhl{\$object}s (a) more, (b) less, or (c) as specified in the input, in terms of a given range of possible \phhl{\$object} values \\
    \hline
...produces \phhl{\$output\_type}s that make the entity producing the text come across to an observer as \phhl{\$property} (a) more, (b) less, or (c) to the degree specified in the input \\
    \hline
...produces \phhl{\$output\_type}s that result in \phhl{\$output\_type}s with \phhl{\$\{more, less\}} \phhl{\$property} in a given  \phhl{\$evaluation\_type} \\
\hline
    \end{tabular}
    \caption{The 16 QC definition templates used in QCET. Each template starts with the words \textit{A better system...} which we omit in each template for brevity.}
    \label{tab:definition_templates}
\end{table*}
 


